One Simple Trick to Fix Your Bayesian Neural Network

One of the most popular estimation methods in Bayesian neural networks (BNN) is mean-field variational inference (MFVI). In this work, we show that neural networks with ReLU activation function induce posteriors, that are hard to fit with MFVI. We provide a theoretical justification for this phenomenon, study it empirically, and report the results of a series of experiments to investigate the effect of activation function on the calibration of BNNs. We find that using Leaky ReLU activations leads to more Gaussian-like weight posteriors and achieves a lower expected calibration error (ECE) than its ReLU-based counterpart.

==> BNN Activation arxiv_arXiv/table.tex <==
\begin{table}[t!]
\centering
\caption{Accuracy and ECE for different architectures, activations and datasets. Leaky stands for Leaky ReLU.}

\begin{tabular}{llrrrr}
\toprule
 & {} & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{ECE} \\
 &  & Leaky & ReLU & Leaky & ReLU \\
Dataset & Model &   &  &   &  \\
\midrule
FMNIST & CONV &  \textbf{0.83} & \textbf{0.83} &  \textbf{0.014} & 0.079 \\
 & 3FC &  \textbf{0.83} & 0.82 &  \textbf{0.033} & 0.106 \\
MNIST & CONV &  \textbf{0.98} & \textbf{0.98} &  \textbf{0.018} & 0.042 \\
 & 3FC &  0.97 & \textbf{0.98} &  \textbf{0.007} & 0.019 \\
\bottomrule
\end{tabular}


\label{tab:comparison}

\end{table}

